Enhancing Mental Health Counseling Support in Bangladesh using Culturally-Grounded Knowledge

Large language models (LLMs) show promise in generating supportive responses for mental health and counseling applications. However, their responses often lack cultural sensitivity, contextual grounding, and clinically appropriate guidance. This work addresses the gap of how to systematically incorporate domain-specific, clinically validated knowledge into LLMs to improve counseling quality. We utilize and compare two approaches, retrieval-augmented generation (RAG) and a knowledge graph (KG)-based method, designed to support para-counselors. Our KG is constructed manually and clinically validated, capturing causal relationships between stressors, interventions, and outcomes, with contributions from multidisciplinary people. We evaluated multiple LLMs in both settings using BERTScore F1 and SBERT cosine similarity, as well as human evaluation across five metrics, which is designed to directly measure the effectiveness of counseling beyond similarity at the surface level. The results show that KG-based approaches consistently improve contextual relevance, clinical appropriateness, and practical usability compared to RAG alone, demonstrating that structured, expert-validated knowledge plays a critical role in addressing LLMs limitations in counseling tasks.

==> sections/dataset.tex <==
\section{Dataset}
\label{sec:dataset}

\subsection{Data Collection}

Our dataset is constructed from a collection of structured counseling case records written in Bangla. Each record documents the demographic characteristics of an individual (e.g., age, sex, occupation, marital status), reported causes of distress, and narrative notes prepared for counseling sessions. The sessions were conducted by para-counselors as part of Sajida Foundation's Community Mental Health Initiative. The cases reflect real-world mental health intake scenarios and thus provide naturalistic descriptions of emotional states, stressors, and behavioral symptoms. Each record consists of 2-6 sessions among the participants and a para-counselor. We also provide a strict guideline to the para-counselors on conducting sessions, which we have discussed in Appendix~\ref{appn:guideline_session}.



%Each session log is summarized by the PWLE, containing structured demographic information, reported concerns, and counseling notes used for subsequent analysis. 
Across all sessions, para-counselors record the participant’s problems, contextual factors (such as family, economic, or social influences), emotional responses, and the interventions or guidance provided. This structured approach ensures that the collected data captures both the counseling process and the evolution of the participant’s situation over time. As a result, we obtained $402$ participant records from Sajida Foundation's Community Mental Health Initiative. Participants vary in age, occupation, marital status, and socioeconomic background, reflecting diverse life circumstances and sources of psychological distress. The records include both short categorical fields (e.g., gender, employment status) and longer narrative descriptions capturing emotional states, perceived causes of stress, and recommended interventions.



\begin{figure*}[t]
\centering
\includegraphics[width=0.9\linewidth]{images/poverty_kg_main_figure_textured.pdf}
\caption{Illustrative subgraph of the knowledge graph used in the KG-based counseling framework. Nodes are grouped into three broad components: poverty drivers, problem states or consequences, and interventions or supports. Directed edges denote four relation types used in the graph: \textit{Causes}, \textit{Leads to}, \textit{Addresses}, and \textit{Mitigates}. For readability, this figure shows only a curated, representative subset of the most salient nodes and relations used in the system, rather than the full knowledge graph. The complete graph is substantially larger and contains additional nodes, edges, and relation instances not displayed here.}
%\vspace{-0.4cm}
\label{fig:poverty-kg}
\end{figure*}

\subsection{Manual Annotation}
Following the annotation guidelines in Appendix~\ref{sec:annotation_guideline}, the manual annotation process was conducted in two structured steps to ensure narrative quality, privacy compliance, and clinical validity. Our pool of manual annotators consists of 6 individuals, including one person with lived experience (PWLE), two public health researchers (PHRs), two Psychologists, and one Psychiatrist. In the first step, annotators %(PWLE and PHRs) 
removed direct identifiers (e.g., names, workplaces, locations) and generalized specific dates using relative session references. This step was carried out collaboratively by one PWLE and two PHRs, who independently reviewed cases and documented suggested corrections before reconciling differences through discussion.

In second step, two licensed psychologists independently evaluated whether the narrative contained sufficient information to establish a meaningful cause and effect relationship, whether protective and risk factors were correctly categorized, and whether the intervention type was clinically appropriate given the participant’s demographics and context. The annotation task was evenly distributed between psychologists. If a psychologist raised concerns about certain cases, particularly regarding the appropriateness of the clinical interpretation, a discussion was arranged among the psychologists and the psychiatrist to reach a final adjudication and resolve discrepancies.  %and provide authoritative guidance. 
This multi-disciplinary annotation framework ensured both methodological rigor and clinical reliability in the final labeled dataset. As a result of the manual annotation process, we obtained a final dataset of 69 individual annotated cases. We provide a detailed analysis of the data in Appendix~\ref{appn:data_analysis}. 




\subsection{Knowledge Graph Construction}
Following manual annotation, the annotated cases were transformed into a structured knowledge graph (KG) to represent relationships among causes, interventions, effects, and outcomes in counseling narratives. The nodes and relationships of KG were selected in a co-design workshop in the presence of PWLE, para-counselors, psychologists, and psychiatrists, ensuring that the relationships reflect clinically meaningful reasoning and domain expertise. Once the KG was built, it was %integrated with our solution, and the generated session guidance was tested with PWLE, Para-counselor, and psychologist. They were also part for validation.
%The validated data were 
migrated into a graph database using relational queries, converting static annotations into a dynamic and traversable relational structure. This process enabled the modeling of causal and intervention pathways within mental health support scenarios.


The resulting knowledge graph contains 308 nodes and 642 relationships across nine relationship types. The structure is dense and multi-dimensional, capturing complex connections between causes, protective factors, interventions, and outcomes in a form that can be systematically explored and analyzed. The nodes represent domain entities such as causes, effects, interventions, outcomes, and conceptual categories, while the edges encode the semantic relationships between them. We provide the detailed statistics of KG in Table~\ref{tab:kg_stats}. Moreover, we provide an overview of the KG with a subset of data in Figure~\ref{fig:poverty-kg}.



\begin{table}[!ht]
\centering
\scalebox{0.8}{
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lrp{4.5cm}}
\toprule
\textbf{Relationship} & \textbf{Count} & \textbf{Connection Logic} \\ \midrule
MITIGATES & 368 & Intervention $\rightarrow$ Effect \\
LEADS\_TO & 184 & Intervention $\rightarrow$ Outcome \\
CAUSES & 92 & Cause $\rightarrow$ Effect \\
ADDRESSES & 92 & Intervention $\rightarrow$ Cause \\
BELONGS\_TO & 23 & Node $\rightarrow$ Category \\
COMPLEMENTS & 20 & Intervention $\rightarrow$ Intervention \\
RELATED\_TO & 20 & Node $\rightarrow$ Node \\
EXACERBATES & 14 & Cause $\rightarrow$ Cause \\
REQUIRES & 9 & Intervention $\rightarrow$ Intervention \\
\bottomrule
\end{tabular}
}
\caption{Relationship distribution of the knowledge graph}
\vspace{-0.4cm}
\label{tab:kg_stats}
\end{table}








==> sections/intro-old.tex <==
\section{Introduction}
\label{sec:introduction}
Mental health systems in developing countries such as Bangladesh remain severely under-resourced, with significant constraints in both financial investment and trained mental health personnel \cite{rahaman2025mental, jahan2024ngos, harrison2019strategic}. In response to these resource constraints, Bangladesh, like many developing nations, has increasingly relied on task-shifting approaches, in which non-specialists, called para-counselors, with minimal training (ranging from several weeks to one month) in basic counseling skills and mental health first aid deliver frontline mental health support \cite{mariam2023sisters}. Evidence suggests that psychological interventions delivered by such para-counselors can be effective in resource-constrained settings \cite{van2013non, singla2023role}. 



\begin{figure}[t]
\centering
%\vspace{-0.4cm}
\includegraphics[width=0.7\linewidth]{latex/images/methodology.png}
\caption{Overview of the methodology incorporating RAG-based experiments.}
\vspace{-0.6cm}
\label{fig:methodology}
\end{figure}

In the context of the present study, para-counselors occupy an intermediary position between community health workers and mental health specialists. Community health workers identify and refer individuals presenting with psychological distress. Para-counselors then conduct a structured series of sessions, typically four to six, depending on the severity and vulnerability of the case. If they identify that a community member needs professional support, they may refer the individual to a psychologist, psychiatrist, or a tele-mental health service \cite{mariam2023sisters}. 

Despite their pivotal role, para-counselors in Bangladesh, like lay counselors and frontline health workers in other developing nations, often operate with minimal supervision, limited refresher training, and limited access to real-time clinical guidance for providing culturally sensitive care \cite{singla2022culturally}. Addressing these systemic limitations is essential to strengthening community mental health care and ensuring that task-shifting models translate into safe, effective, and equitable service delivery. To address these concerns, recent research, though it has not focused on para-counselors particularly, has explored the potential of using LLMs to support frontline health workers in meeting knowledge and decision-support needs \cite{ramjee2025ashabot, moosa2025evaluating, lima2025spotlighting, rutunda2025good, mastel2025mbaza, al2023transforming}. Para-counselors in Bangladesh could benefit from such systems, particularly where access to specialist supervision is limited. 

However, while this body of work acknowledges the possible advantages of LLM-powered tools, it also underscores important ethical and contextual risks \cite{ramjee2025ashabot, lima2025spotlighting}. Scholars suggest that for an effective collaboration between LLM-based systems and healthcare workers to meet frontline health workers' knowledge needs, the models must show a deep understanding of the sociocultural contexts in which they are deployed \cite{ramjee2025ashabot, lima2025spotlighting}. Without such value alignment, LLMs might risk reproducing Western norms and assumptions, potentially imposing culturally incongruent interpretations of distress or overlooking structural issues such as patriarchy and economic precarity \cite{song2025typing, Aleem2024-me}. 

We propose a generative AI support system that augments their capacity in two non-diagnostic ways to address the knowledge-support needs of such para-counselors. First, the system acts as a symptom-reflection and messaging assistant, helping counselors draft context-sensitive responses based on session summaries. Second, it functions as a query-based educational tool, providing real-time guidance on therapeutic strategies and locally grounded idioms of care. To facilitate the effective development of such a system, we investigate two key research questions: \textit{(i)} to what extent do LLMs reflect cultural understandings of mental health when used by para-counselors supporting low-income communities in Bangladesh? and \textit{(ii)} how can LLMs deployed to support lower-income communities in Bangladesh be designed to be more culturally sensitive?

To address these research questions, we first constructed a dataset from initial counseling sessions conducted by para-counselors with lower-income community members and used it within a retrieval-augment generation (RAG) framework to provide contextual grounding for LLMs, given their known limitations in cultural sensitivity \cite{liu2026tailored}. We then developed a culturally grounded knowledge graph (KG) through a co-design process involving para-counselors, persons with lived experience (PWLEs), public health researchers (PHRs), psychologists, and psychiatrists to experiment with the KG-based framework. KG captures causal relationships among triggers, symptoms, and coping strategies (e.g., economic hardship $\rightarrow$ sleep loss $\rightarrow$ perceived spiritual affliction), as well as local idioms of distress, to better ground LLM responses. 

Our findings highlight the importance of socio-technical approaches for improving the cultural sensitivity of the LLM-based knowledge-support system of para-counselors. We found that the LLM with structured knowledge yields significantly better quality and practical relevance than RAG-based models that rely on unstructured data. Further, quantitative evaluations across four language models, assessing fluency, relevance, and cultural alignment, complemented with human evaluations from para-counselors, PHRs, PWLE, psychologists, and psychiatrists, indicate that effective counseling support depends not only on semantic similarity to reference responses but also on clear language, accurate interpretation of concerns, appropriate guidance, and contextual awareness. 




 



